Single versus Multi-Tone Wireless Power Transfer with Physically Large Array

Distributed beamforming is a key enabler to provide power wirelessly to a massive amount of energy-neutral devices (ENDs). However, without prior information and fully depleted ENDs, initially powering these devices efficiently is an open question. This work investigates and assesses the feasibility of harvesting sufficient energy to transmit a backscatter pilot signal from the END, which can be then used for coherent downlink transmission. We experimentally evaluated adaptive single-tone and multi-tone signals during initial charging. The results indicate that the response time for ENDs with unknown locations can extend to several tens of seconds. Notably, the adaptive single-tone excitation shows, among others, better performance at lower transmit power levels, providing a faster response. These findings underscore the potential of adaptive single-tone signals in optimizing power delivery to END in future networks.

==> IEEEabrv.tex <==
journal = IEEE_J_AC,
@STRING{IEEE_J_ANNE = "{IEEE} Trans. Aeronaut. Navig. Electron."}
@STRING{IEEE_J_AES = "{IEEE} Trans. Aerosp. Electron. Syst."}
@STRING{IEEE_J_ANE = "{IEEE} Trans. Aerosp. Navig. Electron."}
@STRING{IEEE_J_AS = "{IEEE} Trans. Aerosp."}
@STRING{IEEE_J_AIRE = "{IEEE} Trans. Airborne Electron."}
@STRING{IEEE_J_MIL = "{IEEE} Trans. Mil. Electron."}
@STRING{IEEE_J_ITS = "{IEEE} Trans. Intell. Transp. Syst."}
@STRING{IEEE_J_IV = "{IEEE} Trans. Intell. Veh."}
@STRING{IEEE_J_TTE = "{IEEE} Trans. Transport. Electrific."}
@STRING{IEEE_J_VC = "{IEEE} Trans. Veh. Commun."}
@STRING{IEEE_J_VT = "{IEEE} Trans. Veh. Technol."}
@STRING{IEEE_J_STSP = "{IEEE} J. Sel. Topics Signal Process."}
@STRING{IEEE_J_SPL = "{IEEE} Signal Process. Lett."}
@STRING{IEEE_J_SYST = "{IEEE} Syst. J."}
@STRING{IEEE_J_ASSP = "{IEEE} Trans. Acoust., Speech, Signal Process."}
@STRING{IEEE_J_AU = "{IEEE} Trans. Audio"}
@STRING{IEEE_J_AUEA = "{IEEE} Trans. Audio Electroacoust."}
@STRING{IEEE_J_ASLP = "{IEEE/ACM} Trans. Audio, Speech, Language Process."}
@STRING{IEEE_J_ASL = "{IEEE} Audio, Speech, Language Process."}
@STRING{IEEE_J_AC = "{IEEE} Trans. Autom. Control"}
@STRING{IEEE_J_CAS = "{IEEE} Trans. Circuits Syst."}
@STRING{IEEE_J_CASVT = "{IEEE} Trans. Circuits Syst. Video Technol."}
@STRING{IEEE_J_CASI = "{IEEE} Trans. Circuits Syst. {I}"}
@STRING{IEEE_J_CASII = "{IEEE} Trans. Circuits Syst. {II}"}
@STRING{IEEE_J_CASI_RP = "{IEEE} Trans. Circuits Syst. {I}"}
@STRING{IEEE_J_CASII_EB = "{IEEE} Trans. Circuits Syst. {II}"}
@STRING{IEEE_J_CT = "{IEEE} Trans. Circuit Theory"}
@STRING{IEEE_J_CST = "{IEEE} Trans. Control Syst. Technol."}
@STRING{IEEE_J_ETCAS = "{IEEE} Trans. Emerg. Sel. Topics Circuits Syst."}
@STRING{IEEE_J_SP = "{IEEE} Trans. Signal Process."}
@STRING{IEEE_J_SU = "{IEEE} Trans. Sonics Ultrason."}
@STRING{IEEE_J_SAP = "{IEEE} Trans. Speech Audio Process."}
@STRING{IEEE_J_UE = "{IEEE} Trans. Ultrason. Eng."}
@STRING{IEEE_J_UFFC = "{IEEE} Trans. Ultrason., Ferroelectr., Freq. Control"}
@STRING{IEEE_J_COML = "{IEEE} Commun. Lett."}
@STRING{IEEE_J_JSAC = "{IEEE} J. Sel. Areas Commun."}
@STRING{IEEE_J_COM = "{IEEE} Trans. Commun."}
@STRING{IEEE_J_COMT = "{IEEE} Trans. Commun. Technol."}
@STRING{IEEE_J_WCOM = "{IEEE} Trans. Wireless Commun."}
@STRING{IEEE_J_WCOML = "{IEEE} Wireless Commun. Lett."}
@STRING{IEEE_J_ADVP = "{IEEE} Trans. Adv. Packag."}
@STRING{IEEE_J_CHMT = "{IEEE} Trans. Compon., Hybrids, Manuf. Technol."}
@STRING{IEEE_J_CPMT = "{IEEE} Trans. Compon. Packag. Manuf. Technol."}
@STRING{IEEE_J_CPMTA = "{IEEE} Trans. Compon., Packag., Manuf. Technol. {A}"}
@STRING{IEEE_J_CPMTB = "{IEEE} Trans. Compon., Packag., Manuf. Technol. {B}"}
@STRING{IEEE_J_CPMTC = "{IEEE} Trans. Compon., Packag., Manuf. Technol. {C}"}
@STRING{IEEE_J_CAPTS = "{IEEE} Trans. Compon. Packag. Technol."}
@STRING{IEEE_J_CAPT = "{IEEE} Trans. Compon. Packag. Technol."}
@STRING{IEEE_J_CPART = "{IEEE} Trans. Compon. Parts"}
@STRING{IEEE_J_EPM = "{IEEE} Trans. Electron. Packag. Manuf."}
@STRING{IEEE_J_MFT = "{IEEE} Trans. Manuf. Technol."}
@STRING{IEEE_J_PHP = "{IEEE} Trans. Parts, Hybrids, Packag."}
@STRING{IEEE_J_PMP = "{IEEE} Trans. Parts, Mater., Packag."}
@STRING{IEEE_J_TCAD = "{IEEE} J. Technol. Comput. Aided Design"}
@STRING{IEEE_J_CAD = "{IEEE} Trans. Comput.-Aided Design Integr. Circuits Syst."}
@STRING{IEEE_J_BD = "{IEEE} Trans. Big Data"}
@STRING{IEEE_J_IFS = "{IEEE} Trans. Inf. Forensics Security"}
@STRING{IEEE_J_IT = "{IEEE} Trans. Inf. Theory"}
@STRING{IEEE_J_KDE = "{IEEE} Trans. Knowl. Data Eng."}
@STRING{IEEE_J_CAL = "{IEEE} Comput. Archit. Lett."}
@STRING{IEEE_J_ES = "{IEEE} Embedded Syst. Lett."}
@STRING{IEEE_J_IOT = "{IEEE} Internet Things J."}
@STRING{IEEE_J_XCDC = "{IEEE} J. Explor. Solid-State Computat. Devices Circuits"}
@STRING{IEEE_J_MMCT = "{IEEE} J. Multiscale and Multiphys. Comput. Techn."}
@STRING{IEEE_J_SUSC = "{IEEE} Sustain. Comput."}
@STRING{IEEE_J_CC = "{IEEE} Trans. on Cloud Comput."}
@STRING{IEEE_J_CSS = "{IEEE} Trans. Comput. Social Syst."}
@STRING{IEEE_J_C = "{IEEE} Trans. Comput."}
@STRING{IEEE_J_CNS = "{IEEE} Trans. Control Netw. Syst."}
@STRING{IEEE_J_DSC = "{IEEE} Trans. Depend. Sec. Comput."}
@STRING{IEEE_J_ECOMP = "{IEEE} Trans. Electron. Comput."}
@STRING{IEEE_J_ETC = "{IEEE} Trans. Emerg. Topics Comput."}
@STRING{IEEE_J_EVC = "{IEEE} Trans. Evol. Comput."}
@STRING{IEEE_J_FUZZ = "{IEEE} Trans. Fuzzy Syst."}
@STRING{IEEE_J_MC = "{IEEE} Trans. Mobile Comput."}
@STRING{IEEE_J_MSCS = "{IEEE} Trans. Multi-Scale Comput. Syst."}
@STRING{IEEE_J_NET = "{IEEE/ACM} Trans. Netw."}
@STRING{IEEE_J_NSE = "{IEEE} Trans. Netw. Sci. Eng."}
@STRING{IEEE_J_NSM = "{IEEE} Trans. Netw. Service Manag."}
@STRING{IEEE_J_NN = "{IEEE} Trans. Neural Netw."}
@STRING{IEEE_J_NNLS = "{IEEE} Trans. Neural Netw. Learn. Syst."}
@STRING{IEEE_J_PDS = "{IEEE} Trans. Parallel Distrib. Syst."}
@STRING{IEEE_J_SC = "{IEEE} Trans. Serv. Comput."}
@STRING{IEEE_J_SIPN = "{IEEE} Trans. Signal Inf. Process. Netw."}
@STRING{IEEE_J_SE = "{IEEE} Trans. Softw. Eng."}
@STRING{IEEE_J_JDT = "{IEEE/OSA} J. Display Technol."}
@STRING{IEEE_J_IP = "{IEEE} Trans. Image Process."}
@STRING{IEEE_J_MM = "{IEEE} Trans. Multimedia"}
@STRING{IEEE_J_VCG = "{IEEE} Trans. Vis. Comput. Graphics"}
@STRING{IEEE_J_JAS = "{IEEE/CAA} J. Autom. Sinica"}
@STRING{IEEE_J_JRA = "{IEEE} J. Robot. Autom."}
@STRING{IEEE_J_AFFC = "{IEEE} Trans. Affect. Comput."}
@STRING{IEEE_J_ASE = "{IEEE} Trans. Autom. Sci. Eng."}
@STRING{IEEE_J_AMD = "{IEEE} Trans. Auton. Mental Develop."}
@STRING{IEEE_J_CCN = "{IEEE} Trans. on Cogn. Commun. Netw."}
@STRING{IEEE_J_CDS = "{IEEE} Trans. Cogn. Develop. Syst."}
@STRING{IEEE_J_CIAIG = "{IEEE} Trans. Comput. Intell. {AI} in Games"}
@STRING{IEEE_J_CYB = "{IEEE} Trans. Cybern."}
@STRING{IEEE_J_H = "{IEEE} Trans. Haptics"}
@STRING{IEEE_J_HFE = "{IEEE} Trans. Hum. Factors Electron."}
@STRING{IEEE_J_HMS = "{IEEE} Trans. Human-Mach. Syst."}
@STRING{IEEE_J_MMS = "{IEEE} Trans. Man-Mach. Syst."}
@STRING{IEEE_J_PAMI = "{IEEE} Trans. Pattern Anal. Mach. Intell."}
@STRING{IEEE_J_RA = "{IEEE} Trans. Robot. Autom."}
@STRING{IEEE_J_RAL = "{IEEE} Robot. Autom. Lett."}
@STRING{IEEE_J_RO = "{IEEE} Trans. Robot."}
@STRING{IEEE_J_SMC = "{IEEE} Trans. Syst., Man, Cybern."}
@STRING{IEEE_J_SMCA = "{IEEE} Trans. Syst., Man, Cybern. {A}"}
@STRING{IEEE_J_SMCB = "{IEEE} Trans. Syst., Man, Cybern. {B}"}
@STRING{IEEE_J_SMCC = "{IEEE} Trans. Syst., Man, Cybern. {C}"}
@STRING{IEEE_J_SMCS = "{IEEE} Trans. Syst., Man, Cybern., Syst."}
@STRING{IEEE_J_SSC = "{IEEE} Trans. Syst. Sci. Cybern."}
@STRING{IEEE_J_GRSL = "{IEEE} Geosci. Remote Sens. Lett."}
@STRING{IEEE_J_GE = "{IEEE} Trans. Geosci. Electron."}
@STRING{IEEE_J_GRS = "{IEEE} Trans. Geosci. Remote Sens."}
@STRING{IEEE_J_OE = "{IEEE} J. Ocean. Eng."}
@STRING{IEEE_J_STARS = "{IEEE} J. Sel. Topics Appl. Earth Observ. Remote Sens."}
@STRING{IEEE_J_CJECE = "Canadian J. Elect. Comput. Eng."}
@STRING{IEEE_J_PROC = "Proc. {IEEE}"}
@STRING{IEEE_J_RITA = "{IEEE} Revista Iberoamericana de Technolog{\'{i}}as del Aprendizaje"}
@STRING{IEEE_J_EDU = "{IEEE} Trans. Educ."}
@STRING{IEEE_J_EM = "{IEEE} Trans. Eng. Manag."}
@STRING{IEEE_J_EWS = "{IEEE} Trans. Eng. Writing Speech"}
@STRING{IEEE_J_LT = "{IEEE} Trans. Learn. Technol."}
@STRING{IEEE_J_PC = "{IEEE} Trans. Prof. Commun."}
@STRING{IEEE_J_AWPL = "{IEEE} Antennas Wireless Propag. Lett."}
@STRING{IEEE_J_MAGL = "{IEEE} Magn. Lett."}
@STRING{IEEE_J_MGWL = "{IEEE} Microw. Guided Wave Lett."}
@STRING{IEEE_J_MWCL = "{IEEE} Microw. Wireless Compon. Lett."}
@STRING{IEEE_J_RFIC = "{IEEE} {RFIC} J."}
@STRING{IEEE_J_RFID = "{IEEE} {RFID} J."}
@STRING{IEEE_J_AP = "{IEEE} Trans. Antennas Propag."}
@STRING{IEEE_J_EMC = "{IEEE} Trans. Electromagn. Compat."}
@STRING{IEEE_J_MAG = "{IEEE} Trans. Magn."}
@STRING{IEEE_J_MTT = "{IEEE} Trans. Microw. Theory Techn."}
@STRING{IEEE_J_RFI = "{IEEE} Trans. Radio Freq. Interference"}
@STRING{IEEE_J_TTHZ = "{IEEE} Trans. {THz} Sci. Technol."}
@STRING{IEEE_J_TJMJ = "{IEEE} Transl. J. Magn. Jpn."}
@STRING{IEEE_J_PHOT = "{IEEE} J. Photovolt."}
@STRING{IEEE_J_PEL = "{IEEE} Power Electron. Lett."}
@STRING{IEEE_J_PETS = "{IEEE} Power Energy Technol. Syst. J."}
@STRING{IEEE_J_ESTPE = "{IEEE} Trans. Emerg. Sel. Topics Power Electron."}
@STRING{IEEE_J_EC = "{IEEE} Trans. Energy Convers."}
@STRING{IEEE_J_PWRAS = "{IEEE} Trans. Power App. Syst."}
@STRING{IEEE_J_PWRD = "{IEEE} Trans. Power Del."}
@STRING{IEEE_J_PWRE = "{IEEE} Trans. Power Electron."}
@STRING{IEEE_J_PWRS = "{IEEE} Trans. Power Syst."}
@STRING{IEEE_J_SG = "{IEEE} Trans. Smart Grid"}
@STRING{IEEE_J_STE = "{IEEE} Trans. Sustain. Energy"}
@STRING{IEEE_J_PSE = "{IEEE} J. Product Safety Eng."}
@STRING{IEEE_J_APPIND = "{IEEE} Trans. Appl. Ind."}
@STRING{IEEE_J_BC = "{IEEE} Trans. Broadcast."}
@STRING{IEEE_J_BCTV = "{IEEE} Trans. Broadcast Television Receivers"}
@STRING{IEEE_J_CE = "{IEEE} Trans. Consum. Electron."}
@STRING{IEEE_J_IE = "{IEEE} Trans. Ind. Electron."}
@STRING{IEEE_J_IECI = "{IEEE} Trans. Ind. Electron. Contr. Instrum."}
@STRING{IEEE_J_IA = "{IEEE} Trans. Ind. Appl."}
@STRING{IEEE_J_IGA = "{IEEE} Trans. Ind. Gen. Appl."}
@STRING{IEEE_J_IINF = "{IEEE} Trans. Ind. Informat."}
@STRING{IEEE_J_IM = "{IEEE} Trans. Instrum. Meas."}
@STRING{IEEE_J_JEM = "{IEEE/TMS} J. Electron. Mater."}
@STRING{IEEE_J_DEI = "{IEEE} Trans. Dielectr. Electr. Insul."}
@STRING{IEEE_J_EI = "{IEEE} Trans. Electr. Insul."}
@STRING{IEEE_J_MEMS = "J. Microelectromech. Syst."}
@STRING{IEEE_J_MEMSI = "J. Microelectromech. Syst."}
@STRING{IEEE_J_MECH = "{IEEE/ASME} Trans. Mechatronics"}
@STRING{IEEE_J_BHI = "{IEEE} J. Biomed. Health Inform."}
@STRING{IEEE_J_TEHM = "{IEEE} J. Transl. Eng. Health Med."}
@STRING{IEEE_J_LS = "{IEEE} Life Sci. Lett."}
@STRING{IEEE_J_RBME = "{IEEE} Rev. Biomed. Eng."}
@STRING{IEEE_J_BCAS = "{IEEE} Trans. Biomed. Circuits Syst."}
@STRING{IEEE_J_BMELC = "{IEEE} Trans. Bio-Med. Electron."}
@STRING{IEEE_J_BME = "{IEEE} Trans. Biomed. Eng."}
@STRING{IEEE_J_B-ME = "{IEEE} Trans. Bio-Med. Eng."}
@STRING{IEEE_J_CBB = "{IEEE/ACM} Trans. Comput. Biol. Bioinformatics"}
@STRING{IEEE_J_ITBM = "{IEEE} Trans. Inf. Technol. Biomed."}
@STRING{IEEE_J_ME = "{IEEE} Trans. Med. Electron."}
@STRING{IEEE_J_MI = "{IEEE} Trans. Med. Imag."}
@STRING{IEEE_J_MBSC = "{IEEE} Trans. Mol. Biol. Multi-Scale Commun."}
@STRING{IEEE_J_NB = "{IEEE} Trans. Nanobiosci."}
@STRING{IEEE_J_NSRE = "{IEEE} Trans. Neural Syst. Rehabil. Eng."}
@STRING{IEEE_J_RE = "{IEEE} Trans. Rehabil. Eng."}
@STRING{IEEE_J_JLT = "J. Lightw. Technol."}
@STRING{IEEE_J_OCN = "{IEEE} J. Opt. Commun. Netw."}
@STRING{IEEE_J_PJ = "{IEEE} Photon. J."}
@STRING{IEEE_J_PTL = "{IEEE} Photon. Technol. Lett."}
@STRING{IEEE_J_EDL = "{IEEE} Electron Device Lett."}
@STRING{IEEE_J_EDS = "{IEEE} J. Electron Devices Soc."}
@STRING{IEEE_J_JQE = "{IEEE} J. Quantum Electron."}
@STRING{IEEE_J_JSTQE = "{IEEE} J. Sel. Topics Quantum Electron."}
@STRING{IEEE_J_ENANO = "{IEEE} Nanotechnol. Express"}
@STRING{IEEE_J_ED = "{IEEE} Trans. Electron Devices"}
@STRING{IEEE_J_NANO = "{IEEE} Trans. Nanotechnol."}
@STRING{IEEE_J_NS = "{IEEE} Trans. Nucl. Sci."}
@STRING{IEEE_J_PS = "{IEEE} Trans. Plasma Sci."}
@STRING{IEEE_J_DMR = "{IEEE} Trans. Device Mater. Rel."}
@STRING{IEEE_J_R = "{IEEE} Trans. Rel."}
@STRING{IEEE_J_ESSL = "{IEEE/ECS} Electrochem. Solid-State Lett."}
@STRING{IEEE_J_JSSC = "{IEEE} J. Solid-State Circuits"}
@STRING{IEEE_J_ASC = "{IEEE} Trans. Appl. Supercond."}
@STRING{IEEE_J_SM = "{IEEE} Trans. Semicond. Manuf."}
@STRING{IEEE_J_SENSOR = "{IEEE} Sensors J."}
@STRING{IEEE_J_VLSI = "{IEEE} Trans. {VLSI} Syst."}
@STRING{IEEE_O_ACC = "{IEEE} Access"}
@STRING{IEEE_M_AES = "{IEEE} Aerosp. Electron. Syst. Mag."}
@STRING{IEEE_M_HIST = "{IEEE} Ann. Hist. Comput."}
@STRING{IEEE_M_AP = "{IEEE} Antennas Propag. Mag."}
@STRING{IEEE_M_ASSP = "{IEEE} {ASSP} Mag."}
@STRING{IEEE_M_CHINAC = "China Commun."}
@STRING{IEEE_M_CD = "{IEEE} Circuits Devices Mag."}
@STRING{IEEE_M_CAS = "{IEEE} Circuits Syst. Mag."}
@STRING{IEEE_M_COM = "{IEEE} Commun. Mag."}
@STRING{IEEE_M_COMSOC = "{IEEE} Commun. Soc. Mag."}
@STRING{IEEE_O_CSTO = "{IEEE} Commun. Surveys Tuts."}
@STRING{IEEE_M_CIM = "{IEEE} Comput. Intell. Mag."}
@STRING{IEEE_M_CSE = "{IEEE} Comput. Sci. Eng."}
@STRING{IEEE_M_CSEM = "{IEEE} Comput. Sci. Eng. Mag."}
@STRING{IEEE_M_C = "Computer"}
@STRING{IEEE_M_CAP = "{IEEE} Comput. Appl. Power"}
@STRING{IEEE_M_CGA = "{IEEE} Comput. Graph. Appl."}
@STRING{IEEE_M_CONC = "{IEEE} Concurrency"}
@STRING{IEEE_M_CS = "{IEEE} Control Syst. Mag."}
@STRING{IEEE_M_DT = "{IEEE} Des. Test"}
@STRING{IEEE_M_DTC = "{IEEE} Des. Test. Comput."}
@STRING{IEEE_O_DSO = "{IEEE} Distrib. Syst. Online"}
@STRING{IEEE_M_EI = "{IEEE} Electr. Insul. Mag."}
@STRING{IEEE_M_ETF = "{IEEE} Electrific. Mag."}
@STRING{IEEE_M_EMC = "{IEEE} Electromagn. Compat."}
@STRING{IEEE_M_ETR = "{IEEE} ElectroTechnol. Rev."}
@STRING{IEEE_M_EMR = "{IEEE} Eng. Manag. Rev."}
@STRING{IEEE_M_EMB = "{IEEE} Eng. Med. Biol. Mag."}
@STRING{IEEE_M_EXP = "{IEEE} Expert"}
@STRING{IEEE_M_GRS = "{IEEE} Geosci. Remote Sens. Mag."}
@STRING{IEEE_M_IA = "{IEEE} Ind. Appl. Mag."}
@STRING{IEEE_M_IE = "{IEEE} Ind. Electron. Mag."}
@STRING{IEEE_M_IM = "{IEEE} Instrum. Meas. Mag."}
@STRING{IEEE_M_IS = "{IEEE} Intell. Syst."}
@STRING{IEEE_M_ITS = "{IEEE} Intell. Transp. Syst. Mag."}
@STRING{IEEE_M_IC = "{IEEE} Internet Comput."}
@STRING{IEEE_M_ITP = "{IEEE} {IT} Prof."}
@STRING{IEEE_M_MICRO = "{IEEE} Micro"}
@STRING{IEEE_M_MW = "{IEEE} Microw. Mag."}
@STRING{IEEE_M_MM = "{IEEE} Multimedia"}
@STRING{IEEE_M_NANO = "{IEEE} Nanotechnol. Mag."}
@STRING{IEEE_M_NET = "{IEEE} Netw."}
@STRING{IEEE_M_PCOM = "{IEEE} Personal Commun. Mag."}
@STRING{IEEE_M_PVC = "{IEEE} Pervasive Comput."}
@STRING{IEEE_M_POT = "{IEEE} Potentials"}
@STRING{IEEE_M_PEL = "{IEEE} Power Electron. Mag."}
@STRING{IEEE_M_PE = "{IEEE} Power Energy Mag."}
@STRING{IEEE_M_PER = "{IEEE} Power Eng. Rev."}
@STRING{IEEE_M_PULSE = "{IEEE} Pulse"}
@STRING{IEEE_M_RA = "{IEEE} Robot. Autom. Mag."}
@STRING{IEEE_M_SAP = "{IEEE} Security Privacy"}
@STRING{IEEE_M_SP = "{IEEE} Signal Process. Mag."}
@STRING{IEEE_M_S = "{IEEE} Softw."}
@STRING{IEEE_M_SSC = "{IEEE} Solid-State Circuits Mag."}
@STRING{IEEE_M_SPECT = "{IEEE} Spectr."}
@STRING{IEEE_M_SMC = "{IEEE} Syst., Man, Cybern. Mag."}
@STRING{IEEE_M_TS = "{IEEE} Technol. Soc. Mag."}
@STRING{IEEE_M_VT = "{IEEE} Veh. Technol. Mag."}
@STRING{IEEE_M_WC = "{IEEE} Wireless Commun."}
@STRING{IEEE_M_TODAY = "Today's Engineer"}


==> bib.tex <==
@inproceedings{10014336,
	title        = {{Simple Transmit-Phase optimization for Focused-Beamforming Wireless Energy Transfer}},
	author       = {Fujii, Masaaki},
	year         = 2022,
	booktitle    = {2022 IEEE 11th Global Conference on Consumer Electronics (GCCE)},
	pages        = {213--214},
	doi          = {10.1109/GCCE56475.2022.10014336}
}
@article{10026518,
	title        = {{Optimal transmit beamforming for near-field integrated sensing and wireless power transfer systems}},
	author       = {Sun, Ping and Dai, Haibo and Wang, Baoyun},
	year         = 2022,
	journal      = {Intelligent and Converged Networks},
	volume       = 3,
	number       = 4,
	pages        = {378--386},
	doi          = {10.23919/ICN.2022.0028}
}
@inproceedings{10283480,
	title        = {{XL-MIMO Channel Modeling and Prediction for Wireless Power Transfer}},
	author       = {Deutschmann, Benjamin J. B. and Wilding, Thomas and Graber, Maximilian and Witrisal, Klaus},
	year         = 2023,
	booktitle    = {2023 IEEE International Conference on Communications Workshops (ICC Workshops)},
	pages        = {1355--1361},
	doi          = {10.1109/ICCWorkshops57953.2023.10283480}
}
@article{7932461,
	title        = {{Low-Complexity Adaptive Multisine Waveform Design for Wireless Power Transfer}},
	author       = {Clerckx, Bruno and Bayguzina, Ekaterina},
	year         = 2017,
	journal      = {IEEE Antennas and Wireless Propagation Letters},
	volume       = 16,
	pages        = {2207--2210},
	doi          = {10.1109/LAWP.2017.2706944}
}
@inproceedings{9814679,
	title        = {{Location-based Initial Access for Wireless Power Transfer with Physically Large Arrays}},
	author       = {Deutschmann, Benjamin J. B. and Wilding, Thomas and Larsson, Erik G. and Witrisal, Klaus},
	year         = 2022,
	booktitle    = {2022 IEEE International Conference on Communications Workshops (ICC Workshops)},
	pages        = {127--132},
	doi          = {10.1109/ICCWorkshops53468.2022.9814679}
}
@article{bolos2016rf,
	title        = {{RF energy harvesting from multi-tone and digitally modulated signals}},
	author       = {Bolos, Ferran and Blanco, Javier and Collado, Ana and Georgiadis, Apostolos},
	year         = 2016,
	journal      = {IEEE Transactions on Microwave Theory and Techniques},
	publisher    = {IEEE},
	volume       = 64,
	number       = 6,
	pages        = {1918--1927}
}
@inproceedings{callebaut2022techtile,
	title        = {{Techtile--open 6G R\&D testbed for communication, positioning, sensing, WPT and federated learning}},
	author       = {Callebaut, Gilles and Van Mulders, Jarne and Ottoy, Geoffrey and Delabie, Daan and Cox, Bert and Stevens, Nobby and Van der Perre, Liesbet},
	year         = 2022,
	booktitle    = {2022 Joint European Conference on Networks and Communications \& 6G Summit (EuCNC/6G Summit)},
	pages        = {417--422},
	organization = {IEEE}
}
@book{chen2019,
	title        = {{Energy harvesting communications: Principles and theories}},
	author       = {Chen, Yunfei},
	year         = 2019,
	publisher    = {John Wiley \& Sons},
	series       = {THEi Wiley ebooks},
	isbn         = {1-119-38308-0},
	edition      = {First edition.},
	language     = {eng},
	owner        = {Thomas Wilding},
	timestamp    = {2024.08.02 10:27}
}
@article{divakaran2019rf,
	title        = {{RF energy harvesting systems: An overview and design issues}},
	author       = {Divakaran, Sleebi K and Krishna, Deepti Das and Nasimuddin},
	year         = 2019,
	journal      = {International Journal of RF and Microwave Computer-Aided Engineering},
	publisher    = {Wiley Online Library},
	volume       = 29,
	number       = 1
}
@misc{github,
	title        = {{Scripts and Data -- Single versus Multi-Tone Wireless Power Transfer with Physically Large Arrays}},
	author       = {Jarne {Van Mulders} and Gilles {Callebaut}},
	year         = 2024,
	journal      = {GitHub repository},
	publisher    = {GitHub},
	howpublished = {\url{https://github.com/techtile-by-dramco/wpt-signals-for-initial-access/}}
}
@article{hajimiriDynamicFocusingLarge2021,
	title        = {{Dynamic Focusing of Large Arrays for Wireless Power Transfer and Beyond}},
	author       = {Hajimiri, Ali and Abiri, Behrooz and Bohn, Florian and {Gal-Katziri}, Matan and Manohara, Mohith H.},
	year         = 2021,
	month        = jul,
	journal      = {IEEE Journal of Solid-State Circuits},
	volume       = 56,
	number       = 7,
	pages        = {2077--2101},
	doi          = {10.1109/JSSC.2020.3036895},
	issn         = {0018-9200, 1558-173X},
	urldate      = {2024-07-16},
	copyright    = {https://creativecommons.org/licenses/by-nc-nd/4.0/},
	langid       = {english},
	file         = {C:\Users\Calle\OneDrive - KU Leuven\Zotero\Hajimiri et al. - 2021 - Dynamic Focusing of Large Arrays for Wireless Powe.pdf}
}
@inproceedings{rajabi2016impact,
	title        = {{Impact of multisine excitation design on rectifier performance}},
	author       = {Rajabi, Mohammad and Pan, Ning and Pollin, Sofie and Schreurs, Dominique},
	year         = 2016,
	booktitle    = {2016 46th European Microwave Conference (EuMC)},
	pages        = {1151--1154},
	organization = {IEEE}
}
@article{shariati2018multitone,
	title        = {{Multitone excitation analysis in RF energy harvesters--Considerations and limitations}},
	author       = {Shariati, Negin and Scott, James R and Schreurs, Dominique and Ghorbani, Kamran},
	year         = 2018,
	journal      = {IEEE Internet of Things Journal},
	publisher    = {IEEE},
	volume       = 5,
	number       = 4,
	pages        = {2804--2816}
}
@inproceedings{SPAWC2,
	title        = {{How to Perform Distributed Precoding to Wirelessly Power Shelf Labels: Signal Processing and Measurements}},
	author       = {Gilles Callebaut and Jarne {Van Mulders} and Bert Cox and Liesbet {Van der Perre} and Lieven {De Strycker} and Fran\c{c}ois Rottenberg},
	year         = 2024,
	month        = sep,
	booktitle    = {2024 IEEE 25th International Workshop on Signal Processing Advances in Wireless Communications (SPAWC) (IEEE SPAWC 2024)},
	address      = {Lucca, Italy},
	pages        = {4.97},
	days         = 8
}
@inproceedings{trotter2009power,
	title        = {{Power-optimized waveforms for improving the range and reliability of RFID systems}},
	author       = {Trotter, Matthew S and Griffin, Joshua D and Durgin, Gregory D},
	year         = 2009,
	booktitle    = {2009 IEEE International Conference on RFID},
	pages        = {80--87},
	organization = {IEEE}
}
@inproceedings{vanmulders2024keepingenergyneutraldevicesoperational,
	title        = {{Keeping Energy-Neutral Devices Operational: a Coherent Massive Beamforming Approach}},
	author       = {Jarne {Van Mulders} and Bert Cox and Benjamin J. B. Deutschmann and Gilles Callebaut and Lieven {De Strycker} and Liesbet {Van der Perre}},
	year         = 2024,
	month        = sep,
	booktitle    = {2024 IEEE 25th International Workshop on Signal Processing Advances in Wireless Communications (SPAWC) (IEEE SPAWC 2024)},
	address      = {Lucca, Italy},
	pages        = {4.97},
	days         = 8
}

@ARTICLE{Lopez21CSIfree-vs-CSIbased,
  author={López, Onel L. A. and Mahmood, Nurul Huda and Alves, Hirley and Latva-aho, Matti},
  journal={IEEE Transactions on Wireless Communications}, 
  title={{CSI}-Free vs {CSI}-Based Multi-Antenna {WET} for Massive Low-Power Internet of Things}, 
  year={2021},
  volume={20},
  number={5},
  pages={3078-3094},
  doi={10.1109/TWC.2020.3047355}}
